Three-dimensional Quantum Supergravity and Supersymmetric Spin Foam Models

We show how super BF theory in any dimension can be quantized as a spin foam model, generalizing the situation for ordinary BF theory. This is a first step toward quantizing supergravity theories. We investigate in particular 3-dimensional (p=1,q=1) supergravity which we quantize exactly. We obtain a super-Ponzano-Regge model with gauge group OSp(1|2). A main motivation for our approach is the implementation of fermionic degrees of freedom in spin foam models. Indeed, we propose a description of the fermionic degrees of freedom in our model. Complementing the path integral approach we also discuss aspects of a canonical quantization in the spirit of loop quantum gravity. Finally, we comment on 2+1-dimensional quantum supergravity and the inclusion of a cosmological constant.

==> figures/fig_2cableid.tex <==
$\rxy{
,(-7,8);(7,8)**\dir{-};(7,-8)**\dir{-}
;(-7,-8)**\dir{-};(-7,8)**\dir{-}
,(-4,12)*{\blacktriangle},(-4,8);(-4,15)**\dir{-}
,(4,12)*{\blacktriangledown},(4,8);(4,15)**\dir{-}
,(-4,-12)*{\blacktriangle},(-4,-8);(-4,-15)**\dir{-}
,(4,-12)*{\blacktriangledown},(4,-8);(4,-15)**\dir{-}
}\quad =\quad
\rxy{
*\cir(4,0){},(0,4)*{\blacktriangleright},(6,4)*{-1}
,(0,12)*\cir(4,0){d_u}
,(0,-12)*\cir(4,0){u_d}
,(-4,12)*{\blacktriangle};(-4,15)**\dir{-}
,(4,12)*{\blacktriangledown};(4,15)**\dir{-}
,(-4,-12)*{\blacktriangle};(-4,-15)**\dir{-}
,(4,-12)*{\blacktriangledown};(4,-15)**\dir{-}
}$

==> figures/fig_add.tex <==
$\rxy{,(0,5)*\cir(3,0){}*{\lambda}
,(0,-5)*\cir(3,0){}*{\mu}
,(0,-13);(0,-8)**\dir{-}
,(0,-2);(0,2)**\dir{-}
,(0,8);(0,13)**\dir{-}
}
\quad = \quad
\rxy{,(0,0)*\cir(5,0){}*{\lambda+\mu}
,(0,-13);(0,-5)**\dir{-}
,(0,5);(0,13)**\dir{-}
}$

==> figures/fig_gaugeid.tex <==
$\rxy{,(0,0)*{\cdots}
,(-1,25);(-1,20)**\dir{-},(1,25);(1,20)**\dir{-}
,(-1,10);(-1,5)**\dir{-},(1,10);(1,5)**\dir{-}
,(-3,20);(3,20)**\dir{-};(3,10)**\dir{-}
;(-3,10)**\dir{-};(-3,20)**\dir{-}
,(-1,-5);(-1,-10)**\dir{-},(1,-5);(1,-10)**\dir{-}
,(-1,-20);(-1,-25)**\dir{-},(1,-20);(1,-25)**\dir{-}
,(-3,-10);(3,-10)**\dir{-};(3,-20)**\dir{-}
;(-3,-20)**\dir{-};(-3,-10)**\dir{-}
,(-11,-5);(-11,-10)**\dir{-},(-9,-5);(-9,-10)**\dir{-}
,(-11,-20);(-11,-25)**\dir{-},(-9,-20);(-9,-25)**\dir{-}
,(-13,-10);(-7,-10)**\dir{-};(-7,-20)**\dir{-}
;(-13,-20)**\dir{-};(-13,-10)**\dir{-}
,(9,-5);(9,-10)**\dir{-},(11,-5);(11,-10)**\dir{-}
,(9,-20);(9,-25)**\dir{-},(11,-20);(11,-25)**\dir{-}
,(7,-10);(13,-10)**\dir{-};(13,-20)**\dir{-}
;(7,-20)**\dir{-};(7,-10)**\dir{-}
,(-17,15);(17,15)**\dir{--};(17,-15)**\dir{--}
;(-17,-15)**\dir{--};(-17,15)**\dir{--}
} \quad = \quad
\rxy{,(0,0)*{\cdots}
,(-1,25);(-1,5)**\dir{-},(1,25);(1,5)**\dir{-}
,(-1,-5);(-1,-10)**\dir{-},(1,-5);(1,-10)**\dir{-}
,(-1,-20);(-1,-25)**\dir{-},(1,-20);(1,-25)**\dir{-}
,(-3,-10);(3,-10)**\dir{-};(3,-20)**\dir{-}
;(-3,-20)**\dir{-};(-3,-10)**\dir{-}
,(-11,-5);(-11,-10)**\dir{-},(-9,-5);(-9,-10)**\dir{-}
,(-11,-20);(-11,-25)**\dir{-},(-9,-20);(-9,-25)**\dir{-}
,(-13,-10);(-7,-10)**\dir{-};(-7,-20)**\dir{-}
;(-13,-20)**\dir{-};(-13,-10)**\dir{-}
,(9,-5);(9,-10)**\dir{-},(11,-5);(11,-10)**\dir{-}
,(9,-20);(9,-25)**\dir{-},(11,-20);(11,-25)**\dir{-}
,(7,-10);(13,-10)**\dir{-};(13,-20)**\dir{-}
;(7,-20)**\dir{-};(7,-10)**\dir{-}
,(-15,15);(15,15)**\dir{--};(15,-15)**\dir{--}
;(-15,-15)**\dir{--};(-15,15)**\dir{--}
}$

==> figures/fig_hkdef.tex <==
$\rxy{(0,13)*{i},(0,-13)*{j},(0,7)*{\blacktriangledown}
,(0,-10);(0,-3)**\dir{-}
,(0,3);(0,10)**\dir{-}
,(0,0)*\cir(3,0){}*{\lambda}
,(3,7)*{V}
}$


==> figures/fig_jump.tex <==
$\rxy{,(-4,6)*\cir(3,0){}*{\lambda}
,(-4,-13);(-4,-7)**\dir{-}
,(-4,1);(-4,3)**\dir{-}
,(-4,9);(-4,13)**\dir{-}
,(4,-13);(4,-7)**\dir{-}
,(4,1);(4,13)**\dir{-}
,(-7,-7);(7,-7)**\dir{-};(7,1)**\dir{-}
;(-7,1)**\dir{-};(-7,-7)**\dir{-}
}
\quad = \quad
\rxy{,(4,6)*\cir(3,0){}*{\lambda}
,(-4,-13);(-4,-7)**\dir{-}
,(-4,1);(-4,13)**\dir{-}
,(4,-13);(4,-7)**\dir{-}
,(4,1);(4,3)**\dir{-}
,(4,9);(4,13)**\dir{-}
,(-7,-7);(7,-7)**\dir{-};(7,1)**\dir{-}
;(-7,1)**\dir{-};(-7,-7)**\dir{-}
}$

==> figures/fig_mat1.tex <==
\rxy{(0,13)*{i},(0,-13)*{j},(0,7)*{\blacktriangledown}
,(0,-10);(0,-4)**\dir{-}
,(0,4);(0,10)**\dir{-}
,(-3,-4);(3,-4)**\dir{-};(3,4)**\dir{-}
;(-3,4)**\dir{-};(-3,-4)**\dir{-}
,(3,7)*{V}
}


==> figures/fig_mat3.tex <==
\rxy{(-7,13)*{i},(-7,-13)*{j},(-7,7)*{\blacktriangledown},(-4,7)*{V}
,(0,13)*{k},(0,-13)*{l},(0,7)*{\blacktriangledown},(3,7)*{W}
,(7,13)*{m},(7,-13)*{n},(7,7)*{\blacktriangle},(10,7)*{X}
,(-7,-10);(-7,-4)**\dir{-}
,(-7,4);(-7,10)**\dir{-}
,(0,-10);(0,-4)**\dir{-}
,(0,4);(0,10)**\dir{-}
,(7,-10);(7,-4)**\dir{-}
,(7,4);(7,10)**\dir{-}
,(-9,-4);(9,-4)**\dir{-};(9,4)**\dir{-}
;(-9,4)**\dir{-};(-9,-4)**\dir{-}
}

==> figures/fig_matid.tex <==
\rxy{(0,13)*{i},(0,-13)*{j},(0,7)*{\blacktriangledown}
,(0,-10);(0,10)**\dir{-}
,(3,7)*{V}}

==> figures/fig_omega.tex <==
\[\rxy{
,(0,-10);(0,10)**\dir{-}
,(2,4)*{\Omega}
}
\quad \defeq \quad \sum_V\quad
\rxy{
,(-12,0)*\cir(4,0){},(-7,-4)*{V}
,(0,-10);(0,10)**\dir{-}
,(2,4)*{V}
}\]

==> figures/fig_sumhk.tex <==
$\rxy{
,(-7,8);(7,8)**\dir{-};(7,-8)**\dir{-}
;(-7,-8)**\dir{-};(-7,8)**\dir{-}
,(-8,8)*\cir(4,0){u_d}
,(-8,-8)*\cir(4,0){d_u}
,(-12,-8);(-12,-3)**\dir{-}
,(-12,3);(-12,8)**\dir{-}
,(0,8);(0,15)**\dir{-}
,(4,8);(4,15)**\dir{-}
,(0,-8);(0,-15)**\dir{-}
,(4,-8);(4,-15)**\dir{-}
,(-12,0)*\cir(3,0){}*{\lambda}
,(-13,-13)*{\Omega}
}\quad =\quad
\rxy{
,(0,-15);(0,-2)**\dir{-}
,(4,-15);(4,-2)**\dir{-}
,(0,2);(0,15)**\dir{-}
,(4,2);(4,15)**\dir{-}
,(2,0)*\cir(3,0){}*{\lambda}
}$

==> figures/fig_sumid.tex <==
$\rxy{
,(-7,8);(7,8)**\dir{-};(7,-8)**\dir{-}
;(-7,-8)**\dir{-};(-7,8)**\dir{-}
,(-8,8)*\cir(4,0){u_d}
,(-8,-8)*\cir(4,0){d_u}
,(-12,-8);(-12,8)**\dir{-}
,(0,8);(0,15)**\dir{-}
,(4,8);(4,15)**\dir{-}
,(0,-8);(0,-15)**\dir{-}
,(4,-8);(4,-15)**\dir{-}
,(-13,-13)*{\Omega}
}\quad =\quad
\rxy{
,(0,-15);(0,15)**\dir{-}
,(4,-15);(4,15)**\dir{-}
}$
